MMLA: Memory-Mediated Learning Architecture for Predictive Dual-State Adaptation

Memory-Mediated Learning Architecture (MMLA) separates slow base parameters theta, a bounded numerical policy carrier Phi, and a bounded authoritative memory M. Predictive Dual-State Adaptation (PDSA) lets feedback update Phi while one problem remains active and lets a trusted lifecycle atomically commit one typed row or exact NULL. Later reasoning may read both states, but their writers, resets, rollback domains, and ledgers remain distinct. Realized futures supervise values only during training; deployment is causal and future-blind. We give conditional theory and falsifiable contracts for reasoning-time updates, completed-segment consolidation, predictive admission, authoritative memory, and dual-state attribution. Assumptions, counterexamples, capacity and cost ledgers, recovery duties, and identifying experiments are explicit; these are not implementation guarantees. Controlled studies show exact lifecycle execution on 300/300 held-out records for each of three seeds, calibrated retrieval gains over frozen-hidden dense and BM25 baselines, and exact typed anchor-filler transport on 240/240 held-out records per seed. These validate restricted components, not natural-language memory management or complete PDSA. Post-training studies retain positive and negative evidence. Later protocols obtain restricted readout progress, but a nine-trajectory comparison finds that matched latent readout, a full-width bridge, and bridge plus frozen text-teacher alignment all fail continuous-event qualification across both task families. A separately adapted text reference and restoration checks pass. At the September 13, 2026 evidence cutoff, no strict policy-only reasoning-time-training effect, predictive-admission oracle margin, learned future-blind admission policy, or policy-by-memory factorial advantage is established.

==> theory_family/modules/amr/preamble.tex <==
% Deterministically namespaced Atomic Memory Rows branch definitions.
\RequirePackage{amsthm}
\RequirePackage{mathtools}
\RequirePackage{bm}
\RequirePackage{longtable}

\newcommand{\tfAmrName}{\textsc{AMR}}
\newcommand{\tfAmrMMLA}{\textsc{MMLA}}
\newcommand{\tfAmrNull}{\textsf{NULL}}
\newcommand{\tfAmrLive}{\textsf{LIVE}}
\newcommand{\tfAmrEmpty}{\textsf{EMPTY}}
\newcommand{\tfAmrTomb}{\textsf{TOMBSTONE}}
\newcommand{\tfAmrQuar}{\textsf{QUARANTINED}}
\newcommand{\tfAmrPass}{\textsf{PASS}}
\newcommand{\tfAmrFail}{\textsf{FAIL}}
\newcommand{\tfAmrUnknown}{\textsf{UNKNOWN}}
\newcommand{\tfAmrCalR}{\mathcal{R}}
\newcommand{\tfAmrCalM}{\mathcal{M}}
\newcommand{\tfAmrCalS}{\mathcal{S}}
\newcommand{\tfAmrCalT}{\mathcal{T}}
\newcommand{\tfAmrCalU}{\mathcal{U}}
\newcommand{\tfAmrCalO}{\mathcal{O}}
\newcommand{\tfAmrCalV}{\mathcal{V}}
\newcommand{\tfAmrCalA}{\mathcal{A}}
\newcommand{\tfAmrCalP}{\mathcal{P}}
\newcommand{\tfAmrE}{\mathbb{E}}
\newcommand{\tfAmrOne}{\mathbf{1}}
\newcommand{\tfAmrBits}{\operatorname{bits}}
\newcommand{\tfAmrSer}{\operatorname{Ser}}
\newcommand{\tfAmrParse}{\operatorname{Parse}}
\newcommand{\tfAmrReplace}{\operatorname{Replace}}
\newcommand{\tfAmrValid}{\operatorname{Valid}}
\newcommand{\tfAmrRead}{\operatorname{Read}}
\newcommand{\tfAmrAuth}{\operatorname{Auth}}
\newcommand{\tfAmrCan}{\operatorname{Can}}
\newcommand{\tfAmrSupp}{\operatorname{supp}_{\mathrm{row}}}
\newcommand{\tfAmrLegal}{\operatorname{Legal}}
\newcommand{\tfAmrTarget}{\operatorname{Target}}
\newcommand{\tfAmrPred}{\operatorname{Pred}}
\newcommand{\tfAmrAssembly}{\operatorname{Assembly}}
\newcommand{\tfAmrLocal}{\operatorname{Local}}
\newcommand{\tfAmrGlobal}{\operatorname{Global}}
\newcommand{\tfAmrReady}{\operatorname{Ready}}

\definecolor{tfAmrNavy}{HTML}{12355B}
\definecolor{tfAmrTeal}{HTML}{008C78}
\definecolor{tfAmrAmber}{HTML}{B96A13}
\definecolor{tfAmrSlate}{HTML}{58677A}
\newcommand{\tfAmrClaimStatus}[2][tfAmrSlate]{\textcolor{#1}{\sffamily\scriptsize\bfseries #2}}
\newcommand{\tfAmrDefinitionStatus}{\tfAmrClaimStatus[tfAmrNavy]{DEFINITION}}
\newcommand{\tfAmrProvedStatus}{\tfAmrClaimStatus[tfAmrTeal]{PROVED UNDER STATED ASSUMPTIONS}}
\newcommand{\tfAmrConjecturedStatus}{\tfAmrClaimStatus[tfAmrAmber]{CONJECTURED}}
\newcommand{\tfAmrPrescriptionStatus}{\tfAmrClaimStatus[tfAmrNavy]{DESIGN PRESCRIPTION}}
\newcommand{\tfAmrPlannedStatus}{\tfAmrClaimStatus[tfAmrAmber]{PLANNED TEST}}
\newcommand{\tfAmrUnvalidatedStatus}{\tfAmrClaimStatus[tfAmrSlate]{UNVALIDATED}}

\theoremstyle{definition}
\newtheorem{tfAmrDefinition}{Definition}[section]
\newtheorem{tfAmrAssumption}[tfAmrDefinition]{Assumption}
\newtheorem{tfAmrProtocol}[tfAmrDefinition]{Protocol}
\newtheorem{tfAmrCounterexample}[tfAmrDefinition]{Counterexample}
\theoremstyle{plain}
\newtheorem{tfAmrLemma}[tfAmrDefinition]{Lemma}
\newtheorem{tfAmrProposition}[tfAmrDefinition]{Proposition}
\newtheorem{tfAmrTheorem}[tfAmrDefinition]{Theorem}
\newtheorem{tfAmrCorollary}[tfAmrDefinition]{Corollary}
\theoremstyle{remark}
\newtheorem{tfAmrRemark}[tfAmrDefinition]{Remark}


==> theory_family/modules/csbc/preamble.tex <==
% Deterministically namespaced completed-segment consolidation definitions.
\RequirePackage{amsthm}
\RequirePackage{mathtools}
\RequirePackage{bm}
\RequirePackage{longtable}

\newcommand{\tfCsbcMMLA}{\textsc{MMLA}}
\newcommand{\tfCsbcName}{\textsc{CSBC}}
\newcommand{\tfCsbcRTT}{\textsc{RTT}}
\newcommand{\tfCsbcRTMA}{\textsc{RTMA}}
\newcommand{\tfCsbcNull}{\textsf{NULL}}
\newcommand{\tfCsbcPass}{\textsf{PASS}}
\newcommand{\tfCsbcFail}{\textsf{FAIL}}
\newcommand{\tfCsbcHold}{\textsf{HOLD}}
\newcommand{\tfCsbcInvalid}{\textsf{INVALID}}
\newcommand{\tfCsbcCalA}{\mathcal{A}}
\newcommand{\tfCsbcCalB}{\mathcal{B}}
\newcommand{\tfCsbcCalC}{\mathcal{C}}
\newcommand{\tfCsbcCalD}{\mathcal{D}}
\newcommand{\tfCsbcCalE}{\mathcal{E}}
\newcommand{\tfCsbcCalF}{\mathcal{F}}
\newcommand{\tfCsbcCalG}{\mathcal{G}}
\newcommand{\tfCsbcCalH}{\mathcal{H}}
\newcommand{\tfCsbcCalI}{\mathcal{I}}
\newcommand{\tfCsbcCalK}{\mathcal{K}}
\newcommand{\tfCsbcCalL}{\mathcal{L}}
\newcommand{\tfCsbcCalM}{\mathcal{M}}
\newcommand{\tfCsbcCalO}{\mathcal{O}}
\newcommand{\tfCsbcCalP}{\mathcal{P}}
\newcommand{\tfCsbcCalQ}{\mathcal{Q}}
\newcommand{\tfCsbcCalR}{\mathcal{R}}
\newcommand{\tfCsbcCalS}{\mathcal{S}}
\newcommand{\tfCsbcCalT}{\mathcal{T}}
\newcommand{\tfCsbcCalU}{\mathcal{U}}
\newcommand{\tfCsbcCalV}{\mathcal{V}}
\newcommand{\tfCsbcCalW}{\mathcal{W}}
\newcommand{\tfCsbcCalX}{\mathcal{X}}
\newcommand{\tfCsbcCalY}{\mathcal{Y}}
\newcommand{\tfCsbcE}{\mathbb{E}}
\newcommand{\tfCsbcP}{\mathbb{P}}
\newcommand{\tfCsbcR}{\mathbb{R}}
\newcommand{\tfCsbcN}{\mathbb{N}}
\newcommand{\tfCsbcOne}{\mathbf{1}}
\newcommand{\tfCsbcGiven}{\,\middle|\,}
\newcommand{\tfCsbcRead}{\operatorname{Read}}
\newcommand{\tfCsbcEmit}{\operatorname{Emit}}
\newcommand{\tfCsbcView}{\operatorname{View}}
\newcommand{\tfCsbcEventize}{\operatorname{Eventize}}
\newcommand{\tfCsbcAnchor}{\operatorname{Anchor}}
\newcommand{\tfCsbcOwner}{\operatorname{Owner}}
\newcommand{\tfCsbcConstruct}{\operatorname{Construct}}
\newcommand{\tfCsbcValidate}{\operatorname{Validate}}
\newcommand{\tfCsbcCommit}{\operatorname{Commit}}
\newcommand{\tfCsbcExpose}{\operatorname{Expose}}
\newcommand{\tfCsbcRetry}{\operatorname{Retry}}
\newcommand{\tfCsbcHash}{\operatorname{Hash}}
\newcommand{\tfCsbcSupp}{\operatorname{supp}_{\rm row}}
\newcommand{\tfCsbcTV}{\operatorname{TV}}

\definecolor{tfCsbcNavy}{HTML}{12355B}
\definecolor{tfCsbcTeal}{HTML}{008C78}
\definecolor{tfCsbcAmber}{HTML}{B96A13}
\definecolor{tfCsbcSlate}{HTML}{58677A}
\definecolor{tfCsbcRed}{HTML}{B83A3A}
\newcommand{\tfCsbcClaimStatus}[2][tfCsbcSlate]{\textcolor{#1}{\sffamily\scriptsize\bfseries #2}}
\newcommand{\tfCsbcDefinitionStatus}{\tfCsbcClaimStatus[tfCsbcNavy]{DEFINITION}}
\newcommand{\tfCsbcProvedStatus}{\tfCsbcClaimStatus[tfCsbcTeal]{PROVED UNDER STATED ASSUMPTIONS}}
\newcommand{\tfCsbcConjecturedStatus}{\tfCsbcClaimStatus[tfCsbcAmber]{CONJECTURED}}
\newcommand{\tfCsbcPrescriptionStatus}{\tfCsbcClaimStatus[tfCsbcNavy]{DESIGN PRESCRIPTION}}
\newcommand{\tfCsbcPlannedStatus}{\tfCsbcClaimStatus[tfCsbcAmber]{PLANNED TEST}}
\newcommand{\tfCsbcUnvalidatedStatus}{\tfCsbcClaimStatus[tfCsbcSlate]{UNVALIDATED}}

\theoremstyle{definition}
\newtheorem{tfCsbcDefinition}{Definition}[section]
\newtheorem{tfCsbcAssumption}[tfCsbcDefinition]{Assumption}
\newtheorem{tfCsbcProtocol}[tfCsbcDefinition]{Protocol}
\newtheorem{tfCsbcCounterexample}[tfCsbcDefinition]{Counterexample}
\theoremstyle{plain}
\newtheorem{tfCsbcLemma}[tfCsbcDefinition]{Lemma}
\newtheorem{tfCsbcProposition}[tfCsbcDefinition]{Proposition}
\newtheorem{tfCsbcTheorem}[tfCsbcDefinition]{Theorem}
\newtheorem{tfCsbcCorollary}[tfCsbcDefinition]{Corollary}
\theoremstyle{remark}
\newtheorem{tfCsbcRemark}[tfCsbcDefinition]{Remark}


==> theory_family/modules/dual_state/preamble.tex <==
% Deterministically namespaced Predictive Dual-State Adaptation branch definitions.
\RequirePackage{amsthm}
\RequirePackage{mathtools}
\RequirePackage{bm}
\RequirePackage{longtable}

\newcommand{\tfDualMMLA}{\textsc{MMLA}}
\newcommand{\tfDualRTT}{\textsc{RTT}}
\newcommand{\tfDualRTMA}{\textsc{RTMA}}
\newcommand{\tfDualNull}{\textsf{NULL}}
\newcommand{\tfDualPass}{\textsf{PASS}}
\newcommand{\tfDualFail}{\textsf{FAIL}}
\newcommand{\tfDualHold}{\textsf{HOLD}}
\newcommand{\tfDualFresh}{\textsf{fresh}}
\newcommand{\tfDualReset}{\textsf{reset}}
\newcommand{\tfDualSwap}{\textsf{swap}}
\newcommand{\tfDualRollback}{\textsf{rollback}}
\newcommand{\tfDualFreeze}{\textsf{freeze}}
\newcommand{\tfDualCalA}{\mathcal{A}}
\newcommand{\tfDualCalC}{\mathcal{C}}
\newcommand{\tfDualCalD}{\mathcal{D}}
\newcommand{\tfDualCalE}{\mathcal{E}}
\newcommand{\tfDualCalF}{\mathcal{F}}
\newcommand{\tfDualCalG}{\mathcal{G}}
\newcommand{\tfDualCalH}{\mathcal{H}}
\newcommand{\tfDualCalI}{\mathcal{I}}
\newcommand{\tfDualCalL}{\mathcal{L}}
\newcommand{\tfDualCalM}{\mathcal{M}}
\newcommand{\tfDualCalO}{\mathcal{O}}
\newcommand{\tfDualCalP}{\mathcal{P}}
\newcommand{\tfDualCalR}{\mathcal{R}}
\newcommand{\tfDualCalS}{\mathcal{S}}
\newcommand{\tfDualCalT}{\mathcal{T}}
\newcommand{\tfDualCalV}{\mathcal{V}}
\newcommand{\tfDualCalW}{\mathcal{W}}
\newcommand{\tfDualCalX}{\mathcal{X}}
\newcommand{\tfDualCalY}{\mathcal{Y}}
\newcommand{\tfDualCalZ}{\mathcal{Z}}
\newcommand{\tfDualE}{\mathbb{E}}
\newcommand{\tfDualP}{\mathbb{P}}
\newcommand{\tfDualR}{\mathbb{R}}
\newcommand{\tfDualOne}{\mathbf{1}}
\newcommand{\tfDualGiven}{\,\middle|\,}
\newcommand{\tfDualDo}{\operatorname{do}}
\newcommand{\tfDualTV}{\operatorname{TV}}
\newcommand{\tfDualVar}{\operatorname{Var}}
\newcommand{\tfDualCov}{\operatorname{Cov}}
\newcommand{\tfDualProj}{\operatorname{proj}}
\newcommand{\tfDualCompat}{\operatorname{Compat}}
\newcommand{\tfDualVerify}{\operatorname{Verify}}
\newcommand{\tfDualRead}{\operatorname{Read}}
\newcommand{\tfDualUpdate}{\operatorname{Update}}
\newcommand{\tfDualCommit}{\operatorname{Commit}}
\newcommand{\tfDualOpReset}{\operatorname{Reset}}
\newcommand{\tfDualOpRollback}{\operatorname{Rollback}}
\newcommand{\tfDualOpSwap}{\operatorname{Swap}}
\newcommand{\tfDualOpSnapshot}{\operatorname{Snapshot}}
\newcommand{\tfDualTrace}{\operatorname{Trace}}
\newcommand{\tfDualCost}{\operatorname{Cost}}
\newcommand{\tfDualPolicy}{\operatorname{Policy}}
\newcommand{\tfDualMemory}{\operatorname{Memory}}
\newcommand{\tfDualGrad}{\nabla}

\definecolor{tfDualNavy}{HTML}{12355B}
\definecolor{tfDualTeal}{HTML}{008C78}
\definecolor{tfDualAmber}{HTML}{B96A13}
\definecolor{tfDualSlate}{HTML}{58677A}
\definecolor{tfDualRed}{HTML}{B83A3A}
\newcommand{\tfDualClaimStatus}[2][tfDualSlate]{\textcolor{#1}{\sffamily\scriptsize\bfseries #2}}
\newcommand{\tfDualDefinitionStatus}{\tfDualClaimStatus[tfDualNavy]{DEFINITION}}
\newcommand{\tfDualProvedStatus}{\tfDualClaimStatus[tfDualTeal]{PROVED UNDER STATED ASSUMPTIONS}}
\newcommand{\tfDualConjecturedStatus}{\tfDualClaimStatus[tfDualAmber]{CONJECTURED}}
\newcommand{\tfDualPrescriptionStatus}{\tfDualClaimStatus[tfDualNavy]{DESIGN PRESCRIPTION}}
\newcommand{\tfDualPlannedStatus}{\tfDualClaimStatus[tfDualAmber]{PLANNED TEST}}
\newcommand{\tfDualUnvalidatedStatus}{\tfDualClaimStatus[tfDualSlate]{UNVALIDATED}}

\theoremstyle{definition}
\newtheorem{tfDualDefinition}{Definition}[section]
\newtheorem{tfDualAssumption}[tfDualDefinition]{Assumption}
\newtheorem{tfDualProtocol}[tfDualDefinition]{Protocol}
\newtheorem{tfDualCounterexample}[tfDualDefinition]{Counterexample}
\theoremstyle{plain}
\newtheorem{tfDualLemma}[tfDualDefinition]{Lemma}
\newtheorem{tfDualProposition}[tfDualDefinition]{Proposition}
\newtheorem{tfDualTheorem}[tfDualDefinition]{Theorem}
\newtheorem{tfDualCorollary}[tfDualDefinition]{Corollary}
\theoremstyle{remark}
\newtheorem{tfDualRemark}[tfDualDefinition]{Remark}


==> theory_family/modules/pma/preamble.tex <==
% Deterministically namespaced Predictive Memory Admission branch definitions.
\RequirePackage{amsthm}
\RequirePackage{mathtools}
\RequirePackage{bm}
\RequirePackage{longtable}

\newcommand{\tfPmaMMLA}{\textsc{MMLA}}
\newcommand{\tfPmaName}{\textsc{PMA}}
\newcommand{\tfPmaNull}{\textsf{NULL}}
\newcommand{\tfPmaPass}{\textsf{PASS}}
\newcommand{\tfPmaFail}{\textsf{FAIL}}
\newcommand{\tfPmaCalA}{\mathcal{A}}
\newcommand{\tfPmaCalD}{\mathcal{D}}
\newcommand{\tfPmaCalE}{\mathcal{E}}
\newcommand{\tfPmaCalF}{\mathcal{F}}
\newcommand{\tfPmaCalG}{\mathcal{G}}
\newcommand{\tfPmaCalH}{\mathcal{H}}
\newcommand{\tfPmaCalI}{\mathcal{I}}
\newcommand{\tfPmaCalL}{\mathcal{L}}
\newcommand{\tfPmaCalM}{\mathcal{M}}
\newcommand{\tfPmaCalO}{\mathcal{O}}
\newcommand{\tfPmaCalR}{\mathcal{R}}
\newcommand{\tfPmaCalS}{\mathcal{S}}
\newcommand{\tfPmaCalW}{\mathcal{W}}
\newcommand{\tfPmaCalX}{\mathcal{X}}
\newcommand{\tfPmaCalZ}{\mathcal{Z}}
\newcommand{\tfPmaE}{\mathbb{E}}
\newcommand{\tfPmaP}{\mathbb{P}}
\newcommand{\tfPmaOne}{\mathbf{1}}
\newcommand{\tfPmaGiven}{\,\middle|\,}
\newcommand{\tfPmaDo}{\operatorname{do}}
\newcommand{\tfPmaTV}{\operatorname{TV}}
\newcommand{\tfPmaVar}{\operatorname{Var}}
\newcommand{\tfPmaCov}{\operatorname{Cov}}
\newcommand{\tfPmaLCB}{\operatorname{LCB}}
\newcommand{\tfPmaUCB}{\operatorname{UCB}}
\newcommand{\tfPmaReg}{\operatorname{Reg}}
\newcommand{\tfPmaValid}{\operatorname{Valid}}
\newcommand{\tfPmaCommit}{\operatorname{Commit}}
\newcommand{\tfPmaConstruct}{\operatorname{Construct}}

\definecolor{tfPmaNavy}{HTML}{12355B}
\definecolor{tfPmaTeal}{HTML}{008C78}
\definecolor{tfPmaAmber}{HTML}{B96A13}
\definecolor{tfPmaSlate}{HTML}{58677A}
\definecolor{tfPmaRed}{HTML}{B83A3A}
\newcommand{\tfPmaClaimStatus}[2][tfPmaSlate]{\textcolor{#1}{\sffamily\scriptsize\bfseries #2}}
\newcommand{\tfPmaDefinitionStatus}{\tfPmaClaimStatus[tfPmaNavy]{DEFINITION}}
\newcommand{\tfPmaProvedStatus}{\tfPmaClaimStatus[tfPmaTeal]{PROVED UNDER STATED ASSUMPTIONS}}
\newcommand{\tfPmaConjecturedStatus}{\tfPmaClaimStatus[tfPmaAmber]{CONJECTURED}}
\newcommand{\tfPmaPrescriptionStatus}{\tfPmaClaimStatus[tfPmaNavy]{DESIGN PRESCRIPTION}}
\newcommand{\tfPmaPlannedStatus}{\tfPmaClaimStatus[tfPmaAmber]{PLANNED TEST}}
\newcommand{\tfPmaUnvalidatedStatus}{\tfPmaClaimStatus[tfPmaSlate]{UNVALIDATED}}

\theoremstyle{definition}
\newtheorem{tfPmaDefinition}{Definition}[section]
\newtheorem{tfPmaAssumption}[tfPmaDefinition]{Assumption}
\newtheorem{tfPmaProtocol}[tfPmaDefinition]{Protocol}
\newtheorem{tfPmaCounterexample}[tfPmaDefinition]{Counterexample}
\theoremstyle{plain}
\newtheorem{tfPmaLemma}[tfPmaDefinition]{Lemma}
\newtheorem{tfPmaProposition}[tfPmaDefinition]{Proposition}
\newtheorem{tfPmaTheorem}[tfPmaDefinition]{Theorem}
\newtheorem{tfPmaCorollary}[tfPmaDefinition]{Corollary}
\theoremstyle{remark}
\newtheorem{tfPmaRemark}[tfPmaDefinition]{Remark}


==> theory_family/modules/rtt/preamble.tex <==
% Deterministically namespaced RTT branch definitions.
\RequirePackage{amsthm}
\RequirePackage{mathtools}
\RequirePackage{bm}
\RequirePackage{longtable}

\newcommand{\tfRttName}{\textsc{RTT}}
\newcommand{\tfRttMemoryAdaptation}{\textsc{RTMA}}
\newcommand{\tfRttTestTimeTraining}{\textsc{TTT}}
\newcommand{\tfRttMMLA}{\textsc{MMLA}}
\newcommand{\tfRttCalF}{\mathcal{F}}
\newcommand{\tfRttCalX}{\mathcal{X}}
\newcommand{\tfRttCalA}{\mathcal{A}}
\newcommand{\tfRttCalO}{\mathcal{O}}
\newcommand{\tfRttCalY}{\mathcal{Y}}
\newcommand{\tfRttCalZ}{\mathcal{Z}}
\newcommand{\tfRttCalC}{\mathcal{C}}
\newcommand{\tfRttCalM}{\mathcal{M}}
\newcommand{\tfRttCalW}{\mathcal{W}}
\newcommand{\tfRttCalP}{\mathcal{P}}
\newcommand{\tfRttCalB}{\mathcal{B}}
\newcommand{\tfRttTV}{\operatorname{TV}}
\newcommand{\tfRttKL}{\operatorname{KL}}
\newcommand{\tfRttE}{\mathbb{E}}
\newcommand{\tfRttP}{\mathbb{P}}
\newcommand{\tfRttInd}{\mathrel{\perp\!\!\!\perp}}
\newcommand{\tfRttGiven}{\,\middle|\,}
\newcommand{\tfRttOne}{\mathbf{1}}

\definecolor{tfRttNavy}{HTML}{12355B}
\definecolor{tfRttTeal}{HTML}{008C78}
\definecolor{tfRttAmber}{HTML}{B96A13}
\definecolor{tfRttSlate}{HTML}{58677A}
\newcommand{\tfRttClaimStatus}[2][tfRttSlate]{\textcolor{#1}{\sffamily\scriptsize\bfseries #2}}
\newcommand{\tfRttDefinitionStatus}{\tfRttClaimStatus[tfRttNavy]{DEFINITION}}
\newcommand{\tfRttAssumptionStatus}{\tfRttClaimStatus[tfRttSlate]{ASSUMPTION}}
\newcommand{\tfRttProvedStatus}{\tfRttClaimStatus[tfRttTeal]{PROVED UNDER STATED ASSUMPTIONS}}
\newcommand{\tfRttConjecturedStatus}{\tfRttClaimStatus[tfRttAmber]{CONJECTURED}}
\newcommand{\tfRttPrescriptionStatus}{\tfRttClaimStatus[tfRttNavy]{DESIGN PRESCRIPTION}}
\newcommand{\tfRttPlannedStatus}{\tfRttClaimStatus[tfRttAmber]{PLANNED TEST}}
\newcommand{\tfRttUnvalidatedStatus}{\tfRttClaimStatus[tfRttSlate]{UNVALIDATED}}

\theoremstyle{definition}
\newtheorem{tfRttDefinition}{Definition}[section]
\newtheorem{tfRttAssumption}[tfRttDefinition]{Assumption}
\newtheorem{tfRttProtocol}[tfRttDefinition]{Protocol}
\newtheorem{tfRttCounterexample}[tfRttDefinition]{Counterexample}
\theoremstyle{plain}
\newtheorem{tfRttLemma}[tfRttDefinition]{Lemma}
\newtheorem{tfRttProposition}[tfRttDefinition]{Proposition}
\newtheorem{tfRttTheorem}[tfRttDefinition]{Theorem}
\newtheorem{tfRttCorollary}[tfRttDefinition]{Corollary}
\theoremstyle{remark}
\newtheorem{tfRttRemark}[tfRttDefinition]{Remark}

